Sundials/ML: Connecting OCaml to the Sundials Numeric Solvers

This paper describes the design and implementation of a comprehensive OCaml interface to the Sundials library of numeric solvers for ordinary differential equations, differential algebraic equations, and non-linear equations. The interface provides a convenient and memory-safe alternative to using Sundials directly from C and facilitates application development by integrating with higher-level language features, like garbage-collected memory management, algebraic data types, and exceptions. Our benchmark results suggest that the interface overhead is acceptable: the standard examples are rarely twice as slow in OCaml than in C, and often less than 50% slower. The challenges in interfacing with Sundials are to efficiently and safely share data structures between OCaml and C, to support multiple implementations of vector operations and linear solvers through a common interface, and to manage calls and error signalling to and from OCaml. We explain how we overcame these difficulties using a combination of standard techniques such as phantom types and polymorphic variants, and carefully crafted data representations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{101}
\providecommand{\publicationstatus}{Kenichi Asai and Mark Shinwell (Eds.)\\
ML/OCaml 2016\\
EPTCS 285, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.285.4}{10.4204/EPTCS.285.4}}
\pdfoutput=1

